Chat More If You Like: Dynamic Cue Words Planning to Flow Longer Conversations

To build an open-domain multi-turn conversation system is one of the most interesting and challenging tasks in Artificial Intelligence. Many research efforts have been dedicated to building such dialogue systems, yet few shed light on modeling the conversation flow in an ongoing dialogue. Besides, it is common for people to talk about highly relevant aspects during a conversation. And the topics are coherent and drift naturally, which demonstrates the necessity of dialogue flow modeling. To this end, we present the multi-turn cue-words driven conversation system with reinforcement learning method (RLCw), which strives to select an adaptive cue word with the greatest future credit, and therefore improve the quality of generated responses. We introduce a new reward to measure the quality of cue words in terms of effectiveness and relevance. To further optimize the model for long-term conversations, a reinforcement approach is adopted in this paper. Experiments on real-life dataset demonstrate that our model consistently outperforms a set of competitive baselines in terms of simulated turns, diversity and human evaluation.

==> reserve/4-simulation.tex <==
\section{Model Training}
\label{training}
%In this section, we present the detailed training process of our model. 
  To warm up for policy model, we firstly fit our model to human-human conversational patterns with supervised learning. Then, through the simulated dialogues between two agents, we optimize the policy model with reinforcement learning. 


  \begin{algorithm}[t]
      \caption{Training Process}
      \label{trainingprocess}
      \begin{algorithmic}[1]
      \State $N$: number of training instances.
      \State $T$: simulation turns.
      \State $M$: sampling times.
      \State Jointly pre-train policy model and cue word augmented response generation model with supervised learning.
       \For {$i=1...N$}
          \State $s_{i,1}=\textsc{Enc}(Q_i)$;
          \For {$m=1...M$}
            \For {$j=1...T$}
                \State Sample an action $a_{i,j}$ based on $s_{i,j}$
                \State Compute $r_{i,j}$ using Eq.~\ref{reward}
                \State Transform to state $s_{i,j+1}$
            \EndFor
            \State Estimate $\mathbb{E}\left[r\left(a_{i,1}, s_{i,1}\right)\right]$ using Eq.~\ref{expectedreward}
          \EndFor
          \State Compute average reward $b_{i,1}$
          \State Update policy model $\mathcal{P}$ using Eq.~\ref{gradient}.
       \EndFor
      \end{algorithmic}
  \end{algorithm}

  \subsection{Single-turn Supervised Learning} 
  \label{supervised}
  For the first stage of training, we aim to learn the cue word augmented response generation model. Given an aligned $\left\langle \textsc{Query}, \textsc{Response}\right\rangle$ pair, we sample a noun, a verb, or an adjective in the reply as the golden cue word $cw$ (See Section~\ref{dataset} for details.). Formally, given the training data $\mathcal{D}=\left\lbrace(Q_1, R_1, {cw}_1),...,(Q_N, R_N, {cw}_N)\right\rbrace$, we formulate the generation model $\mathcal{G}$ as
  \begin{equation}
  \begin{aligned}
  \mathcal{G}(R_i) = p(R_i\mid Q_i, \hat{cw}_i),
  \end{aligned}
  \end{equation}
  where $\hat{cw}_i$ refers to the selected cue word with the highest probability over cue words vocabulary, i.e., $\hat{cw}_i=\argmax_{cw_i} p(cw_i|Q_i)$. Note that $p(cw_i|Q_i)$ here is different from the stochastic policy function $p(a_{i,j}|s_{i,j})$, since the latter one is the policy optimized for long-term future reward.

  The objective function is to minimize the cross entropy of $\mathcal{D}$:
  \begin{equation}
  \begin{aligned}
  -\sum_{i=1}^{N}\left[cw_{i}\log p(\hat{cw}_{i}) + \sum_{k=1}^{m}y_{i,k}\log p(\hat{y}_{i,k})\right]
  \end{aligned}
  \end{equation}
  where $N$ is the number of training instances; $m$ denotes the length of reply words. $cw_i$ and $y_{i,k}$ are the onehot representation of golden cue word and $k$-th word in reply $R_i$, respectively.

  \subsection{Conversation Simulation} 
  The simulation process between two conversational agents consists of following steps: 1) An initial message from training data is fed to agent A as input. 2) Agent A samples a cue word based on the policy model, which computes the probability distribution over cue words vocabulary. 3) Given dialogue context and the selected cue word, agent A generates a response. 4) Transform to new dialogue state, which is fed to agent B as input. 5) Repeat from step 2) to 4) until a conversation reaches an end. 

  %The same as ~\cite{li2016deep}, 
  We define the maximum simulation turns to terminate the simulation process. During the simulation, we optimize the parameters of policy model to improve the probability of an action with a greater expected reward. 



\begin{table}[t]
  \centering
  %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{cc} \hline
    \toprule[0.5pt]
      Number of sessions & $162,143$ \\
      Average number of turns & $6.79$ \\
      Vocabulary Size & $32,979$ \\
      Average length of utterances & $7.79$ \\ 
    \bottomrule[0.5pt]
    \end{tabular}%
  %} 
  \caption{Statistics of the Weibo dataset after filtering.}
  \label{statistics}   
\end{table}

  \subsection{Optimization}
  \label{optimization}
  Results from the supervised model mentioned above will be used to initialize the policy model. Then we use policy gradient~\cite{williams1992simple} for optimization. The objective of learning is to maximize the expected future reward:
  \begin{equation}
   %\mathcal{J}\left(\theta\right)=\sum_{i=1}^{N}\mathop{\mathbb{E}}[r(a_{i,1},s_{i,1})]
  \mathcal{J}\left(\theta\right)=\mathop{\mathbb{E}_{data\sim \mathcal{D}, a_{\cdot,1}\sim \mathcal{P}}}[r(a_{\cdot,1},s_{\cdot,1})]
  \end{equation}
  
  The gradient of objective function is calculated by REINFORCE algorithm~\cite{williams1992simple}:
  \begin{equation}
  \small
  \begin{aligned}
    \nabla_{\theta}\left(\mathcal{J}\right) \approx \frac{1}{N}\sum_{i=1}^{N}\nabla_{\theta}\log p\left(a_{i,1}|s_{i,1}\right)\cdot \\(\sum_{k=1}^{T}r_{i,k}\cdot\gamma^{k-1}-b_{i,1})
  \end{aligned}
  \label{gradient}
  \end{equation}

  where $b_{i,1}$, the average reward of different sampling actions in the same state $s_{i,1}$, is a bias estimator to reduct variance:
  \begin{equation}
	b_{i,1}=\frac{1}{M}\sum_{m=1}^{M}r(a_{i,1}^{m},s_{i,1})
  \end{equation}
  where $a_{i,1}^{m}$ is the $m$-th sampling action in the same state $s_{i,1}$. Together with supervised learning, the whole training process is summarized in Algorithm~\ref{trainingprocess}.




==> reserve/6-results.tex <==
\section{Results and Discussion}

\subsection{Main results}
\textbf{Automatic evaluation.} As shown in Table~\ref{diversity}, our proposed RLCw model significantly outperforms baselines in simulation turns, which demonstrates more active engagement of our method. Table~\ref{diversity} presents the diversity results of all methods. As we see, our proposed RLCw model generates more diverse outputs; it obtains the highest ratio of distinct tri-gram in both intra- and inter-session level. Besides, our RLCw model is slightly inferior to baselines in Dist-1 metric, mainly because of more simulation turns. 
% We argue that there are much more distinct uni-gram (18.92) in a dialogue session, common words such as ``I'' are necessary and inevitable in a longer conversation~\footnote{Based on the statistics, only most frequent 1,492 words can cover 80\% words in training data.}.

Among them, the performance of S2S model is not as good as others. S2S-Cw is slightly inferior to RL-S2S model. However, it generates more distinct words in all simulated conversations comparing with RL-S2S model, as the augmented cue words provide it a broader space for learning. Our proposed RLCw model absorbs its advantage actively and flows a longer and more diverse conversation.


We also provided ablation study result in Table~\ref{diversity}. We can see that \textit{RLCw-Effectiveness} (only use effectiveness reward) method performs not very well in all metrics, mainly because of lacking constraint on reply generation quality. Result of \textit{RLCw-Relevance} is very close to \textit{RLCw}, even surpasses it in terms of diversity. But our \textit{RLCw} still has an advantage in simulation turns, suggesting that using both rewards in training can strengthen our model in terms of user engagement.

\textbf{Human evaluation.} we randomly sample 150 messages from test data to conduct a pairwise comparison, i.e., given a input message, we group two simulated dialogues together\footnote{For fairness, two simulated conversations are pooled and randomly permuted.} and ask the evaluators to choose which is better. We invited four native speakers to offer a judgment. The results of human evaluation against all baseline methods are listed in Table~\ref{casestudy}. Similar to the automatic evaluation results, RLCw consistently outperforms other baselines, which demonstrates the effectiveness of our proposed method. Especially, our proposed method shows significant improvement in term of informativeness and overall popularity.


\subsection{Analysis}
We have elaborated the overall performance of all methods in the last section. Next we will look closer into how cue words affect the dialogue process. 

\textbf{Cue words analysis.} First, we measure the quality and impact of the generated cue words sequence. We try to estimate the quality based on the average cosine similarity of each word pair in the cue words sequence. The result is 0.096 (the correlation of extracted cue words from reply sentences in training data is 0.137), which shows the semantic compactness of them. Again, we use embedding-based metric~\cite{liu2016not} to estimate the correlations between a cue word and the corresponding generated response. The correlation score is 0.81. As we found that there are about 41\% cue words appearing in the simulated dialogues, the selected cue words have a great impact on response generation.

\textbf{Case study.} We further present two representative examples of our generated dialogues in Table~\ref{casestudy}. In the first example, our system dynamically plans a fluent dialogue flow. Based on selected cue words, our RLCw model generates coherent and interesting dialogues. In the second example, our system firstly responds to the given input message, and then shift the topic to ``beauty'' with cue words augmentation, which further affects the direction of the follow-up dialogues.

\textbf{Error analysis.} To gain a deeper understanding of the limitation of our system, we manually reviewed 100 input messages and the corresponding generated dialogues to conduct error analysis. The major problem we found is that the dominant cue words result in irrelevant responses. Although the selected cue word is relevant to dialogue context, the reply seems to fit the cue word well but not the current dialogue state. For example, given the input message ``can I ask what is this countdown for?'', the system predicts a cue word ``ask'' and generates a response ``I'm asking where are you''.  We suspect the decoder concentrates too much on the first layer (green square in Figure~\ref{generation}) in such encoder-decoder framework (sharing parameters with each other).






==> reserve/caogao.tex <==
人机对话系统有广泛的应用***，研究对话系统很必要。 \NoteNP{下面这段可以借鉴，但是要修改}
Conversational robot is one of the most interesting and challenging
topics in artificial intelligence research. It is usually developed to imitate the human-human chatting and applied to many scenarios, such as chitchat, interactive question answering, task-oriented dialogue, interactive recommendation, etc. 
然而开放领域的对话系统研究仍是一个非常有挑战性的问题，目前的研究成果经常出现万能回复，生成句子简短的问题（这里引用Li的文章）。为了解决这个问题，有三个类别的方法：1）***2）*** 3）*** （这里就可以把几个文章放在一起讲，不用像related work那样每个都详细展开）我们是属于第三类。

第二段：然而第三类的两个文章中都规定一个特定measurement 比如PMI指标来选择一个Top 1关键词，然后结合这个关键词来生成回复。但是有时候选出来的Top N个都是很相关的，但不代表选择Top 1就能产生更好的回复。因为对于一个query，可以针对多个aspect进行回答，而对不同的aspect得到的回答可能有不同的效果，即用户并不买账。（show table case），多个aspect，但是有一个是比较好的，或者说有一个人家愿意和你继续聊的。所以说选择一个合适的aspect来回答是很重要的。

第三段：Driven by these, we focus在如何选择某一个aspect进行回答，能给使得对话更多轮，聊天的质量更高，生成句子更加丰富，更像人说话。

%As suggested in ~\cite{vijayakumar2016diverse}, diverse beam search as an alternative to BS is proposed for decoding diverse outputs for a diversity-augmented objective. 
%Modifying standard beam search by expanding penalizing hypotheses of the same parent is suggested in ~\cite{li2016simple}. This algorithm especially contributes to those needing re-ranking. 
%~\newcite{zhou2017mechanism} improved conversation system by developing an encoder-diverter-decoder framework based on the hypotheses about existing latent responding mechanisms. 

%To tackle this issue, prior studies have focused on modifying the loss function~\cite{li2015diversity}, improving the beam search algorithm~\cite{vijayakumar2016diverse,li2016simple,shao2017generating} and  learning latent variables~\cite{zhao2017learning,zhou2017mechanism} to generate diverse responses for a input query.

%As shown in ~\cite{mou2016sequence,yao2017towards,xing2016topic}, better topic should be given by extracting other features provided to the models as conditionals. Inspired by these, we focus on incorporating appropriate information to make an artistic conversation. However, they do not consider the user's feedback during conversation and the generated responses are not up to the actual artistic conversation scenes. The additional information based on a measurement, such as Point-wise Mutual Information (PMI) or twitter LDA topic model, is not adaptive to the artistic dialogue session. Intuitively, given a user-issued query, there may exist many valid responses, each corresponding to a certain aspect from the query. As shown in Table 1\NoteNP{TODO}, these responses derived from different aspects are associated with the query, but the effect varies greatly. Therefore, to select an appropriate aspect is important. 

%\subsection{Reinforcement Learning}
%Reinforcement learning has been a widely used method to solve the problem of decision making. It is a common learning framework through interacting with environment. We will introduce the application of reinforcement learning in text generation and conversation system. 
%In \textit{text generation}, Guo \textit{et al.}~\shortcite{guo2015generating} introduced a novel schema learning with a DQN(Deep Q-Network) for the generating of actions and difficult decoded sequence portions. Mixed Incremental Cross-Entropy Reinforce is proposed to make sequence prediction~\cite{ranzato2015sequence}, with incremental learning and a loss function combining both reinforce and cross entropy~\cite{li2017deep}.  Bahdanau \textit{et al.}~\shortcite{bahdanau2016actor} improved upon Ranzato \textit{et al.}~\shortcite{ranzato2015sequence} by utilizing a critic network with some techniques, such as SARSA, target network, sampling prediction from a delayed actor and reward shaping to predict the value of a token~\cite{li2017deep}. Li \textit{et al.}~\shortcite{li2017learning} took advantage of the knowledge about the future for sequence generation~\cite{li2017deep}.
